COLA: Characterizing and Optimizing the Tail Latency for Safe Level-4 Autonomous Vehicle Systems

Autonomous vehicles (AVs) are envisioned to revolutionize our life by providing safe, relaxing, and convenient ground transportation. The computing systems in such vehicles are required to interpret various sensor data and generate responses to the environment in a timely manner to ensure driving safety. However, such timing-related safety requirements are largely unexplored in prior works. In this paper, we conduct a systematic study to understand the timing requirements of AV systems. We focus on investigating and mitigating the sources of tail latency in Level-4 AV computing systems. We observe that the performance of AV algorithms is not uniformly distributed -- instead, the latency is susceptible to vehicle environment fluctuations, such as traffic density. This contributes to burst computation and memory access in response to the traffic, and further leads to tail latency in the system. Furthermore, we observe that tail latency also comes from a mismatch between the pre-configured AV computation pipeline and the dynamic latency requirements in real-world driving scenarios. Based on these observations, we propose a set of system designs to mitigate AV tail latency. We demonstrate our design on widely-used industrial Level-4 AV systems, Baidu Apollo and Autoware. The evaluation shows that our design achieves 1.65 X improvement over the worst-case latency and 1.3 X over the average latency, and avoids 93% of accidents on Apollo.

==> Makefile <==
.DEFAULT_GOAL:=paper
make_flag:=--no-print-directory -j8

.PHONY: paper
paper:	paper.pdf

paper.pdf: figure
	latexmk -shell-escape -pdf paper.tex
	pdffonts paper.pdf | tee paper.pdf.font.log

.PHONY: grammar
grammar:
	bash script/text_process/pandoc_latex_to_plain.sh paper.tex paper.txt

figure/Makefile: figure/plots.csv \
                 script/figure/configure.py
	@echo GEN $@
	@python script/figure/configure.py gen-makefile $< $@


figure/plots.tex: figure/plots.csv \
                  script/figure/configure.py
	@echo GEN $@
	@python script/figure/configure.py gen-texfile $< $@


.PHONY: figure
figure: figure/Makefile figure/plots.tex
	@make ${make_flag} -C figure all_tikz_pdf all_pdf


.PHONY: clean
clean:
	@latexmk -c

.PHONY: clean_all
clean_all: clean
	@make ${make_flag} -C figure clean


==> config/ieee/bib/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> config/utils.tex <==
% [fh][fh]Figure:
%   [full|half] width [full|half] height figure
\newcommand{\figfullwidth}{7in}
\newcommand{\fighalfwidth}{3.374in}

\newcommand{\figfullheight}{2.69in}
\newcommand{\fighalfheight}{1.8in}

% For tabularx
\newcolumntype{P}{>{\raggedleft\arraybackslash}X}

\newcommand{\squishlist}{
   \begin{list}{$\bullet$}{%
        \setlength{\itemsep}{0pt}%
        \setlength{\parsep}{0pt}%
        \setlength{\topsep}{-3pt}%
        \setlength{\partopsep}{0pt}%
        \setlength{\listparindent}{-2pt}%
        \setlength{\itemindent}{-5pt}%
        \setlength{\leftmargin}{1em}%
        \setlength{\labelwidth}{0em}%
        \setlength{\labelsep}{0.5em}%
    }
}

\newcommand{\squishend}{
    \end{list}  }

\newcommand{\para}[1]{\vspace{0pt}\noindent\textbf{#1}}

\newcommand*\mycircinternal[1]{%
  \tikz[baseline=(char.base)]{%
  \node[minimum size=0.325cm,shape=circle,draw,inner sep=0.25pt,fill=black,text=white,font=\bfseries] (char) {\small#1};}%
\newcommand*\mycirc[1]{%
\raisebox{.5pt}{\mycircinternal{\raisebox{-.9pt} {#1}}}%
}}

% Check mark and cross mark
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

\newboolean{publicversion}
\newboolean{revisedversion}
\newboolean{draftreviewversion}
\setboolean{publicversion}{true}
\setboolean{revisedversion}{false}
\setboolean{draftreviewversion}{false}

% Don't use `todonote` package, it slows down the LaTeX compilation

\ifthenelse{\boolean{publicversion}}{
    \newcommand{\haolan}[1]{}
    \newcommand{\zixuan}[1]{}
    \newcommand{\jishen}[1]{}
    \newcommand{\ignore}[1]{}
    \newcommand{\updatelater}[1]{\PackageError{napaper}{Do NOT use \\updatelater for public version!}}

    \setboolean{revisedversion}{false}
}{
    \newcommand{\draftversion}{1}
    \newcommand{\haolan}[1]{{\color{red}\sf\bfseries\footnotesize Haolan: #1}}
    \newcommand{\zixuan}[1]{{\color{violet}\sf\bfseries\footnotesize Zixuan: #1}}
    \newcommand{\jishen}[1]{{\color{magenta}\sf\bfseries\footnotesize Jishen: #1}}
    \newcommand{\ignore}[1]{{\color{gray}\sf #1}}
    \newcommand{\updatelater}[1]{{\color{blue}#1}}

    \ifthenelse{\boolean{draftreviewversion}}{
        \renewcommand{\haolan}[1]{}
        \renewcommand{\zixuan}[1]{}
        \renewcommand{\jishen}[1]{}
        \renewcommand{\ignore}[1]{}
        \renewcommand{\updatelater}[1]{}
    }{}

    % For date time print
    \edef\pdfilemoddate#1{\pdfcreationdate}
    \usepackage[useregional]{datetime2}
    \usepackage{background}
    \backgroundsetup{color=gray,
                     position=current page.west,
                     angle=90,
                     nodeanchor=west,
                     vshift=-5mm,
                     hshift=-20mm,
                     opacity=1,
                     scale=1.75,
                     contents=DRAFT [Ver.{\draftversion}] {\DTMnow}
    }
}

\ifthenelse{\boolean{revisedversion}}{
    % Highlight for rervision (good with lines that contain \cite{} and \ref{}
    \usepackage{soul, color}
    \soulregister\cite7
    \soulregister\ref7
    \soulregister\pageref7

    % https://tex.stackexchange.com/questions/282386/make-soul-highlight-span-lines
    \makeatletter
    \def\SOUL@hlpreamble{%
        \setul{\dp\strutbox}{\dimexpr\ht\strutbox+\dp\strutbox\relax}%
        \let\SOUL@stcolor\SOUL@hlcolor
        \SOUL@stpreamble
    }
    \makeatother

    % Usage: \st{for paragraph with deleting lines}.}
    % \hl{highlight a paragraph with yellow background.}
    % \renewcommand{\st}[1]{}
} {
    \newcommand{\st}[1]{\PackageError{napaper}{Do NOT use \\st for public version!}}
    \newcommand{\hl}[1]{#1}
    % \newcommand{\hl}[1]{\PackageError{napaper}{Do NOT use \\hl for public version!}}
}


==> figure/Makefile <==

# This Makefile is generated by script/figure/configure.py
# Do not modify this file manually, modify the config file instead

.DEFAULT_GOAL:=all_tikz_pdf

make_flag:=--no-print-directory -j8

RSCRIPT:=Rscript --no-save --no-restore

plot/perf-localization-lidar.tikz: ../data/perf-localization-lidar.csv \
                                   src/perf-localization-lidar.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/perf-localization-lidar.tikz.pdf: plot/perf-localization-lidar.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/perf-prediction-planning.tikz: ../data/perf-prediction-planning.csv \
                                    src/perf-prediction-planning.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/perf-prediction-planning.tikz.pdf: plot/perf-prediction-planning.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/perf-lookahead-distance.tikz: ../data/perf-lookahead-distance.csv \
                                   src/perf-lookahead-distance.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/perf-lookahead-distance.tikz.pdf: plot/perf-lookahead-distance.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/llc-lat-miss.tikz: ../data/llc-lat-miss.csv \
                        src/llc-lat-miss.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/llc-lat-miss.tikz.pdf: plot/llc-lat-miss.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/cpu-util-bursty.tikz: ../data/cpu-util-bursty.csv \
                           src/cpu-util-bursty.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/cpu-util-bursty.tikz.pdf: plot/cpu-util-bursty.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/lat-breakdown-pred-pipeline.tikz: ../data/lat-breakdown-pred-pipeline.csv \
                                       src/lat-breakdown-pred-pipeline.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/lat-breakdown-pred-pipeline.tikz.pdf: plot/lat-breakdown-pred-pipeline.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/lat-fast-normal-path.tikz: ../data/lat-fast-normal-path.csv \
                                src/lat-fast-normal-path.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/lat-fast-normal-path.tikz.pdf: plot/lat-fast-normal-path.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/degradation-rate-alertness.tikz: ../data/degradation-rate-alertness.csv \
                                      src/degradation-rate-alertness.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/degradation-rate-alertness.tikz.pdf: plot/degradation-rate-alertness.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/tail-latency-proactive-processing.tikz: ../data/tail-latency-proactive-processing.csv \
                                             src/tail-latency-proactive-processing.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/tail-latency-proactive-processing.tikz.pdf: plot/tail-latency-proactive-processing.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/lat-dist-before-after-opt.tikz: ../data/lat-dist-before-after-opt.csv \
                                     src/lat-dist-before-after-opt.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/lat-dist-before-after-opt.tikz.pdf: plot/lat-dist-before-after-opt.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/perf-util-bst-effort.tikz: ../data/perf-util-bst-effort.csv \
                                src/perf-util-bst-effort.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/perf-util-bst-effort.tikz.pdf: plot/perf-util-bst-effort.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/perf-improvement-cola.tikz: ../data/perf-improvement-cola.csv \
                                 src/perf-improvement-cola.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/perf-improvement-cola.tikz.pdf: plot/perf-improvement-cola.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/perf-improvement-cola-autoware.tikz: ../data/perf-improvement-cola-autoware.csv \
                                          src/perf-improvement-cola.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/perf-improvement-cola-autoware.tikz.pdf: plot/perf-improvement-cola-autoware.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/crash-cases.tikz: ../data/crash-cases.csv \
                       src/crash-cases.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/crash-cases.tikz.pdf: plot/crash-cases.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/crash-cases-autoware.tikz: ../data/crash-cases-autoware.csv \
                                src/crash-cases.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/crash-cases-autoware.tikz.pdf: plot/crash-cases-autoware.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/driving-time.tikz: ../data/driving-time.csv \
                        src/driving-time.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/driving-time.tikz.pdf: plot/driving-time.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/lat-study-modules.tikz: ../data/lat-study-modules.csv \
                             src/lat-study-modules.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/lat-study-modules.tikz.pdf: plot/lat-study-modules.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/e2e-latency-traffic.tikz: ../data/e2e-latency-traffic.csv \
                               src/e2e-latency-traffic.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/e2e-latency-traffic.tikz.pdf: plot/e2e-latency-traffic.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/reaction-time.tikz: ../data/reaction-time.csv \
                         src/reaction-time.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/reaction-time.tikz.pdf: plot/reaction-time.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


plot/violation.tikz: ../data/violation.csv \
                     src/violation.R
	@echo -e "GEN \t $@"
	@${RSCRIPT} $(word 2,$^) --data $< --out $@ --type tikz 


plot/violation.tikz.pdf: plot/violation.tikz
	@echo -e "GEN \t $@"
	@bash ../script/figure/tikz_to_pdf/tikz_to_pdf.sh $<


./Rplots.svg: ./Rplots.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/util.svg: ./fig/util.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/traffic.svg: ./fig/traffic.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/tf_density.svg: ./fig/tf_density.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/taillatency.svg: ./fig/taillatency.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/sync_overhead.svg: ./fig/sync_overhead.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/sync_improve.svg: ./fig/sync_improve.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/stealing.svg: ./fig/stealing.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/safety_eval.svg: ./fig/safety_eval.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/reduce.svg: ./fig/reduce.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/perception-pipeline.svg: ./fig/perception-pipeline.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/pc.svg: ./fig/pc.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/overall.svg: ./fig/overall.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/memcpy.svg: ./fig/memcpy.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/lookahead.svg: ./fig/lookahead.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/gpuiso.svg: ./fig/gpuiso.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/gpu_kernel.svg: ./fig/gpu_kernel.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/fallback_pred.svg: ./fig/fallback_pred.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/extra.svg: ./fig/extra.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/degrade.svg: ./fig/degrade.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/city.svg: ./fig/city.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/cachemiss_3.svg: ./fig/cachemiss_3.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/bursty.svg: ./fig/bursty.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/all_perf.svg: ./fig/all_perf.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/acc.svg: ./fig/acc.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/autoware_perf.svg: ./fig/autoware_perf.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/autoware_safety_eval.svg: ./fig/autoware_safety_eval.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


./fig/reaction.svg: ./fig/reaction.pdf
	@echo -e "GEN \t $@"
	@bash ../script/figure/pdf_to_svg/pdf_to_svg.sh $<


.PHONY: all
all: all_tikz     \
     all_pdf      \
     all_tikz_pdf \
     all_tikz_svg \
     all_pdf_svg

.PHONY: all_pdf
all_pdf: 

.PHONY:   all_tikz
all_tikz: plot/perf-localization-lidar.tikz           \
          plot/perf-prediction-planning.tikz          \
          plot/perf-lookahead-distance.tikz           \
          plot/llc-lat-miss.tikz                      \
          plot/cpu-util-bursty.tikz                   \
          plot/lat-breakdown-pred-pipeline.tikz       \
          plot/lat-fast-normal-path.tikz              \
          plot/degradation-rate-alertness.tikz        \
          plot/tail-latency-proactive-processing.tikz \
          plot/lat-dist-before-after-opt.tikz         \
          plot/perf-util-bst-effort.tikz              \
          plot/perf-improvement-cola.tikz             \
          plot/perf-improvement-cola-autoware.tikz    \
          plot/crash-cases.tikz                       \
          plot/crash-cases-autoware.tikz              \
          plot/driving-time.tikz                      \
          plot/lat-study-modules.tikz                 \
          plot/e2e-latency-traffic.tikz               \
          plot/reaction-time.tikz                     \
          plot/violation.tikz

.PHONY:       all_tikz_pdf
all_tikz_pdf: plot/perf-localization-lidar.tikz.pdf           \
              plot/perf-prediction-planning.tikz.pdf          \
              plot/perf-lookahead-distance.tikz.pdf           \
              plot/llc-lat-miss.tikz.pdf                      \
              plot/cpu-util-bursty.tikz.pdf                   \
              plot/lat-breakdown-pred-pipeline.tikz.pdf       \
              plot/lat-fast-normal-path.tikz.pdf              \
              plot/degradation-rate-alertness.tikz.pdf        \
              plot/tail-latency-proactive-processing.tikz.pdf \
              plot/lat-dist-before-after-opt.tikz.pdf         \
              plot/perf-util-bst-effort.tikz.pdf              \
              plot/perf-improvement-cola.tikz.pdf             \
              plot/perf-improvement-cola-autoware.tikz.pdf    \
              plot/crash-cases.tikz.pdf                       \
              plot/crash-cases-autoware.tikz.pdf              \
              plot/driving-time.tikz.pdf                      \
              plot/lat-study-modules.tikz.pdf                 \
              plot/e2e-latency-traffic.tikz.pdf               \
              plot/reaction-time.tikz.pdf                     \
              plot/violation.tikz.pdf

.PHONY: all_tikz_svg
all_tikz_svg: 

.PHONY:      all_pdf_svg
all_pdf_svg: ./Rplots.svg                   \
             ./fig/util.svg                 \
             ./fig/traffic.svg              \
             ./fig/tf_density.svg           \
             ./fig/taillatency.svg          \
             ./fig/sync_overhead.svg        \
             ./fig/sync_improve.svg         \
             ./fig/stealing.svg             \
             ./fig/safety_eval.svg          \
             ./fig/reduce.svg               \
             ./fig/perception-pipeline.svg  \
             ./fig/pc.svg                   \
             ./fig/overall.svg              \
             ./fig/memcpy.svg               \
             ./fig/lookahead.svg            \
             ./fig/gpuiso.svg               \
             ./fig/gpu_kernel.svg           \
             ./fig/fallback_pred.svg        \
             ./fig/extra.svg                \
             ./fig/degrade.svg              \
             ./fig/city.svg                 \
             ./fig/cachemiss_3.svg          \
             ./fig/bursty.svg               \
             ./fig/all_perf.svg             \
             ./fig/acc.svg                  \
             ./fig/autoware_perf.svg        \
             ./fig/autoware_safety_eval.svg \
             ./fig/reaction.svg

config: 
	ln -s ../config $@


figure: 
	ln -s . $@


.PHONY:      tikz_to_pdf
tikz_to_pdf: out/plots.pdf

out/plots.pdf: plots.tex                                   \
               config                                      \
               figure                                      \
               plot/perf-localization-lidar.tikz           \
               plot/perf-prediction-planning.tikz          \
               plot/perf-lookahead-distance.tikz           \
               plot/llc-lat-miss.tikz                      \
               plot/cpu-util-bursty.tikz                   \
               plot/lat-breakdown-pred-pipeline.tikz       \
               plot/lat-fast-normal-path.tikz              \
               plot/degradation-rate-alertness.tikz        \
               plot/tail-latency-proactive-processing.tikz \
               plot/lat-dist-before-after-opt.tikz         \
               plot/perf-util-bst-effort.tikz              \
               plot/perf-improvement-cola.tikz             \
               plot/perf-improvement-cola-autoware.tikz    \
               plot/crash-cases.tikz                       \
               plot/crash-cases-autoware.tikz              \
               plot/driving-time.tikz                      \
               plot/lat-study-modules.tikz                 \
               plot/e2e-latency-traffic.tikz               \
               plot/reaction-time.tikz                     \
               plot/violation.tikz
	@latexmk -pdf -outdir=out -quiet plots.tex


.PHONY:clean
clean: clean_tikz     \
       clean_tikz_pdf \
       clean_tikz_svg \
       clean_pdf      \
       clean_symlinks

.PHONY: clean_tikz
clean_tikz: 
	rm -f plot/perf-localization-lidar.tikz plot/perf-prediction-planning.tikz plot/perf-lookahead-distance.tikz plot/llc-lat-miss.tikz plot/cpu-util-bursty.tikz plot/lat-breakdown-pred-pipeline.tikz plot/lat-fast-normal-path.tikz plot/degradation-rate-alertness.tikz plot/tail-latency-proactive-processing.tikz plot/lat-dist-before-after-opt.tikz plot/perf-util-bst-effort.tikz plot/perf-improvement-cola.tikz plot/perf-improvement-cola-autoware.tikz plot/crash-cases.tikz plot/crash-cases-autoware.tikz plot/driving-time.tikz plot/lat-study-modules.tikz plot/e2e-latency-traffic.tikz plot/reaction-time.tikz plot/violation.tikz
	rm -f *_ras1.png


.PHONY: clean_tikz_pdf
clean_tikz_pdf: 
	rm -f plot/perf-localization-lidar.tikz.pdf plot/perf-prediction-planning.tikz.pdf plot/perf-lookahead-distance.tikz.pdf plot/llc-lat-miss.tikz.pdf plot/cpu-util-bursty.tikz.pdf plot/lat-breakdown-pred-pipeline.tikz.pdf plot/lat-fast-normal-path.tikz.pdf plot/degradation-rate-alertness.tikz.pdf plot/tail-latency-proactive-processing.tikz.pdf plot/lat-dist-before-after-opt.tikz.pdf plot/perf-util-bst-effort.tikz.pdf plot/perf-improvement-cola.tikz.pdf plot/perf-improvement-cola-autoware.tikz.pdf plot/crash-cases.tikz.pdf plot/crash-cases-autoware.tikz.pdf plot/driving-time.tikz.pdf plot/lat-study-modules.tikz.pdf plot/e2e-latency-traffic.tikz.pdf plot/reaction-time.tikz.pdf plot/violation.tikz.pdf


.PHONY: clean_tikz_svg
clean_tikz_svg: 
	rm -f 


.PHONY: clean_pdf
clean_pdf: 
	rm -f 

.PHONY: clean_symlinks
clean_symlinks: 
	rm -f config figure

